Ticket-BERT: Labeling Incident Management Tickets with Language Models

An essential aspect of prioritizing incident tickets for resolution is efficiently labeling tickets with fine-grained categories. However, ticket data is often complex and poses several unique challenges for modern machine learning methods: (1) tickets are created and updated either by machines with pre-defined algorithms or by engineers with domain expertise that share different protocols, (2) tickets receive frequent revisions that update ticket status by modifying all or parts of ticket descriptions, and (3) ticket labeling is time-sensitive and requires knowledge updates and new labels per the rapid software and hardware improvement lifecycle. To handle these issues, we introduce Ticket- BERT which trains a simple yet robust language model for labeling tickets using our proposed ticket datasets. Experiments demonstrate the superiority of Ticket-BERT over baselines and state-of-the-art text classifiers on Azure Cognitive Services. We further encapsulate Ticket-BERT with an active learning cycle and deploy it on the Microsoft IcM system, which enables the model to quickly finetune on newly-collected tickets with a few annotations.

==> sections/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\subsection{Text Representation}

Text representation leverages computational methods to transform text into vectors that serve as features for machine learning \cite{hotho2005brief, babic2020survey}. Work focusing on extracting useful information from text comes primarily from three fields: weighted words, word embedding, and linguistic features \cite{revina2020ticket}. The most common weighted features are Bag-of-Words (BoW) \cite{wallach2006topic} and TF-IDF \cite{joachims1996probabilistic}, which represent words as explainable one-hot-encoded vectors; unfortunately, these representations cannot fully capture the word semantics in the context. Word embedding \cite{selva2021review} addresses this limitation by considering word occurrence and co-occurrence. Specifically, each word is represented as a learned vector that conveys information from surrounding words. The representative word embedding methods include Word2Vec \cite{mikolov2013efficient}, GloVe \cite{pennington2014glove}, FastText \cite{bojanowski2017enriching}, and contextualized word representations \cite{levy2014neural,sarzynska2021detecting}. In addition to word embedding, linguistic features are also useful. For example, synonymy and hypernymy are effective methods to increase variants of the text; thus, they can be used as features to measure the text diversity \cite{xiang2014linguistic}. Recent research on linguistic features are described in \cite{revina2020ticket}, such as \cite{revina2021designing} that uses parts-of-speech (PoS) to count tags and conducts ticket classification. However, existing word embedding and linguistic feature methods are not applicable to ticket labeling tasks for the following reasons: $\left(1\right)$ pre-trained word embedding models are not trained on the ticket-related vocabulary containing issue-specific words, and $\left(2\right)$ extracting linguistic features requires input text to be either well-structured or have rich semantic indicators \cite{zhuge2010interactive} whereas ticket descriptions usually have a large amount of unstructured text (e.g., code comments, database queries, cornerstones from different engineers regarding the ticket issues). To address these issues, we apply simple yet effective TF-IDF and BoW features in the baseline models and only use clean text as input for Ticket-BERT models.   



\subsection{Ticket Labeling}
Ticket labeling is the task of assigning specific labels to a given ticket which provides an informative overview of the incident issues therein. General ticket labeling can be done with rule-based methods and machine learning methods: $\left(1\right)$ rule-based methods develop a set of rules to determine ticket labels, such as keyword searching \cite{kim1992fast} or regular expression matching \cite{sidhu2001fast}. These methods are favored by their transparency, explainability, and simplicity \cite{hadi2018integrating, yao2019clinical}. Additionally, rule-based methods can be integrated into machine learning approaches, such as decision trees that develop multiple rules to determine tree splitting \cite{ye2003train, phetrungnapha2019classification}. Note that rule-based ticket labeling may work well on a small set of rules, such as the keywords that address one incident may also apply to another, but could have reduced efficiency when handling a large number of diverse tickets governed by more complex rules. $\left(2\right)$ machine learning methods have demonstrated effectiveness on multiple classification tasks \cite{ikonomakis2005text}. For example, \cite{antoniol2008bug} shows that machine learning methods have advantages to discriminate bugs from incident issues. \cite{herzig2013s} develops machine learning classifiers for identifying incident issues and reveals that developers and maintainers often assign wrong categories to the tickets due to potential intervention from implicit unstructured data (e.g., implicit ticket description addressing an incident issue). To improve this, \cite{zhou2016combining} introduces an ensemble method that leverages both structured and unstructured data to reduce the noise of misclassification via a multi-stage classification approach. However, it is challenging to determine the best machine learning algorithm for a particular application \cite{revina2020ticket} in real-world scenarios. To address these issues, we elected to build end-to-end deep learning language models that avoid the manual creation of complicated rules and feature engineering preprocessing yet achieve state-of-the-art performance for the ticket labeling task.

\subsection{Deep Language Models}

Recently, deep learning methods have gained unprecedented prevalence in natural language processing (NLP) \cite{ikonomakis2005text, parvat2017survey}. For example, Long short-term memory (LSTM) models  \cite{hochreiter1997long} have been trained to solve sequence tagging \cite{huang2015bidirectional}, semantic parsing \cite{xiao2016sequence}, sentiment analysis \cite{huang2016modeling}, and text generation \cite{santhanam2020context}. With regard to text representation, \cite{sarzynska2021detecting} proposes the Embedding from Language Models (ELMo) that learns word vectors by a bidirectional LSTM, where weighted layers are combined as embedding to represent text. Although ELMo has bidirectional neurons that look forward and backward in the text sequence, it is unable to take advantage of both contexts simultaneously, thus its ability to understand text content is limited. To improve this, \cite{devlin2018bert} proposes another Bidirectional Encoder Representations based on Transformers (BERT) that addresses Masked Language Model (MLM) and Next Sentence Prediction (NSP) tasks for training language models. Previous work leverages BERT to conduct classification in computer vision and NLP \cite{sun2019fine, adhikari2019docbert, li2020does, bao2021beit}, and achieved excellent results; however, there is no prior work, to the best of our knowledge, that employs pre-trained BERT models to conduct ticket labeling because ticket data is often domain-specific, complex, and there exists no large-scale labeled datasets publicly available. Smaller datasets may be scraped in individual cases, but several reasons exist as to why these are often not enough to fine-tune a large transformer like BERT. First, ticket data is combination of machine-generated text and natural language. BERT was pre-trained on the latter, and may require more data to learn the nuisances of fragmented text (sometimes even in table format) generated by machines. Second, we observe that some tickets are information sparse, which means that we have a set of hard-to-identify labels. This is one of the reasons why we believe the model would need an active learning cycle [\ref{fig:active_learning}]. In this work, we develop the first TicketBERT for ticket labeling using our proposed datasets. Nevertheless, directly fine-tuning large language models on the dataset (i,e, D-Machine, D-Human, and D-Mixture) that share different vocabulary (e.g., ticket-related tokens) may not perform well. Ticket text uses domain-specific words and/or abbreviations to present incident issues. To solve for this, we borrow the idea from prompt learning \cite{liu2021pre} that helps language models learn factual knowledge \cite{petroni2019language}, and develop novel training strategies to improve ticket labeling performance with language models. Specifically, we take the title and summary as prompt-prefix and concatenate to ticket description. This simple yet effective strategy greatly boosts ticket labeling performance on the difficult D-Human dataset.

